Bulk topological signatures of a quasicrystal

We show how measuring real space properties such as the charge density in a quasiperiodic system can be used to gain insight into their topological properties. In particular, for the Fibonacci chain, we show that the total onsite charge oscillates when plotted in the appropriate coordinates, and the number of oscillations is given by the Chern number of the gap in which the Fermi level lies. We show that these oscillations have two distinct interpretations, obtained by extrapolating results from the two extreme limits of the Fibonacci chain -- the valence bond picture in the strong modulation limit, and perturbation around the periodic chain in the weak modulation limit. This effect is found to remain robust at moderate interactions, as well as in the presence of disorder. We conclude that experimental measurement of the real space charge distribution can yield information on topological properties in a straightforward way.

==> SuppMatTextOnly.tex <==
\section{Spectral analysis using RG in the strong modulation limit}

In the main text, we presented a procedure that recovers the charge density profile in the strong modulation limit, using an RG scheme in real space. In this limit, the band structure and the wave functions are well described in terms of a perturbative RG scheme where the small parameter is the coupling ratio, $\rho=t_A/t_B \ll 1$. Here, we present an alternate equivalent formulation focusing on the splitting of the spectrum.
 
 For $\rho=0$ the chain breaks up into molecules ($m$) and atoms ($a$), and the spectrum consists of three levels that broaden into three bands as $\rho$ is increased. The RG theory gives the relationship between spectra of a long chain and those of shorter chains. Thus one can show that the energy spectrum of the $n$th approximant has a symmetric structure due to the particle-hole symmetry. \footnote{This symmetry is broken when PBC are applied in odd-length chains but is restored in the limit of infinite system size}. One gets three main groups of levels: the lowest $F_{n-2}$ $m$ levels being the so-called molecular bonding ($m_-$), the highest $F_{n-2}$ being antibonding $m_+$) levels. The central group of $F_{n-3}$ levels are so-called atomic ($a$) levels. Each of these can be subdivided into three groups and so on. 

For sites in the conumbering system, the same demarcation occurs within the interval $[1,F_n]$. The first set of $F_{n-2}$ sites (the left subinterval) are $m$ sites and their partners lie in the right subinterval. The $a$ sites lie in the middle subinterval. Filling up the lowest levels results in a charge of 0.5 per $m$ site, filling up all the $a$ levels results in a charge of 1 per $a$ site. 
The p-h symmetry ensures that, for half-filling, all sites are filled equally, with $n_i=0.5$.  

With this notation in place we can now discuss the way total charge is built up on each site for different fillings.
$N_e$ in the following denotes the number of (spinless electrons). One can restrict to the lower half of the spectrum since the upper half can be deduced by p-h symmetry.
Let us consider the cases where $N_e$ is a Fibonacci number, $N_e=F_{n-j}$, where $j=2,3,...$. For any $j$, it is easy to check that $F_{n-j-1}=\mathrm{Mod}[q F_{n-1},F_n]$ with $q=(-1)^j F_{j}$. In other words, all the levels of the lowest band are completely filled upto the gap of label $q$.
\begin{enumerate}
\item For $N_e=F_{n-2}$ ($q=-1$), the lowest band ($m_-$) is completely filled. To leading order, the total charge is $0.5$ on $m$ sites, and 0 on $a$ sites. Plotted as a function of conumber one has a plateau where $n_i = 0.5$ on the left and on the right, and a central region $n_i = 0$. This zero order picture is modified by higher order corrections in $\rho$, that lead to finer structures within each region.  
\item For $N_e=F_{n-4}$ ($q=-3$), the lowest sub-band of the lowest band is completely filled.  This implies that each of the plateaus again splits into two plateaus. The number of maxima (Nb.half-maxima at each edge) is $2^2-1=3$ as expected from the $q$ value for this filling. 
% Upon generalizing to $N_e=F_{n-2j}$, one sees that in the strong modulation limit, certain peaks are vanishingly small. Consider for example $N_e=F_{n-6}$ ($q=-8$). The RG picture one predicts that each of the previous plateaux splits into 2, giving $2^3-1=7$ maxima, plus one in the central region of $a$. The peak in the center is much smaller than the others when $r\rightarrow 0$ but becomes appreciable for intermediate values as shown in Fig.~\ref{fig:Charge-density}.
\item For $N_e=F_{n-3}$ ($q=2$) the lowest band is partly filled, leading to different charges on the two types of $m$ sites. The total onsite occupancy is 0.25 for the $mm$ sites and 0.5 for the $am$ sites to leading order. These values are modified by higher order corrections when $\rho$ is sslowly turned on.
\end{enumerate}
When $N_e$ is not a Fibonacci number, we employ Zeckendorf's theorem in an analogous way to the previous section. Consider for example the case $N_e=F_{n-2}+F_{n-5}$, where one can check that $q=4$. Now the lowest band being completely filled, all of the $m$ sites have a charge of $0.5$. In addition, the occupancy $n_i$ equal to 0.5 at lowest order at the $am$ atom sites (atom sites which become $m$ after an RG step) and their partners to the right. For finite $\rho$, the resulting profile has 4 maxima.
 
The above special cases show how oscillations of charge can be explained based on the simplified picture in the strong modulation limit. 
\section{Perturbative analysis in the weak modulation limit}
When the modulation is weak, $t_A/t_B\sim 1$, we can treat the Fibonacci modulation as a perturbation to the homogeneous chain \cite{sireExcitationSpectrumExtended1990, sireSpectrum1DQuasicrystals1989}. In real space, the Fibonacci hopping Hamiltonian splits into two parts,
\begin{align}
    \hat{H} =& \underbrace{- \sum_{i=1}^{F_n} t_A c^\dagger_i c_{i+1} + h.c.}_{\hat{H}_0}
    \underbrace{- \sum_{i=1}^{F_n} (t_i - t_A) c^\dagger_i c_{i+1} + h.c.}_{\hat{H}_w}
\end{align}
$\hat{H}_0$ is the Hamiltonian of a periodic chain with nearest neighbor hopping $t_A$, and $\hat{H}_w$ introduces the Fibonacci modulation. We use periodic boundary conditions, so the index $i$ (and $j$ in the following) are understood to wrap around modulo $F_n$. The matrix representation of the Fibonacci hopping Hamiltonian in perpendicular space, which we will denote with $\hat{\mathcal{H}}$ has a particularly pleasing form. The only non-zero hopping terms lie on four diagonals. The $-t_A$s go in the $\pm F_{n-2}$th diagonal and the $-t_B$s go in the $\pm F_{n-1}$th diagonal.

The decomposition of $\hat{\mathcal{H}}$ as a sum of a term that represents the homogeneous chain $\hat{\mathcal{H}}_0$ and the Fibonacci perturbation $\hat{\mathcal{H}}_w$ takes the following form:
\begin{align}
    \hat{\mathcal{H}}_0 &= -\sum_{j=1}^{F_n} t_A c_j^\dagger c_{j+F_{n-2}} + t_A c_j^\dagger c_{j+ F_{n-1}} + h.c. \label{eq:H0_perp:S}\\
    \hat{\mathcal{H}}_w &= -\sum_{j=1}^{F_{n-2}} 2w c_j^\dagger c_{j+F_{n-1}} + h.c. \label{Hw_perp:S}
\end{align}
where we have used $2w = t_A-t_B$. $\hat{\mathcal{H}}_w$ connects each of the leftmost $F_{n-2}$ sites to the site $F_{n-1}$ places to its right. $\hat{\mathcal{H}}_0$ is a circulant matrix  and $\hat{\mathcal{H}}_w$ is a Toeplitz matrix with only the $\pm F_{n-1}$th diagonals filled.

Before applying the Fibonacci modulation, consider the eigenstates of the unperturbed Hamiltonian. Recall that the eigenvalues of $\hat{H}_0$ are given by $E_m = -2t_{A}\cos\left(\frac{2\pi m}{F_{n}}\right)$ with the integer $m$ constrained by $0\leq m \leq \lfloor F_n/2\rfloor$. Almost all of these are doubly degenerate. If $F_n$ is odd, the $m=0$ eigenvalue is non-degenerate. If $F_n$ is even, then addditionally, the $m = \lfloor F_n/2 \rfloor$ eigenvalue is also  non-degenerate. The corresponding eigenstates take the form of plane waves with wavenumber $\frac{2\pi}{F_n}m$. 

Remarkably, the unperturbed Hamiltonian represented in perpendicular space is a circulant matrix. This means that it is also diagonalized by a Fourier transformation and the eigenstates, which are plane waves in real space, are also plane waves in perpendicular space. But the wavenumbers are shuffled or the wavenumber that corresponds to a plane wave with a given energy is different. In perpendicular space, the eigenstates are plane waves labelled by the integer $\mu = 0,1,\ldots \lfloor F_n/2\rfloor$. As in real space, the eigenstates are almost all doubly degenerate, and the eigenstate with label $\mu$ has the wavenumber $\frac{2\pi}{F_n}\mu$. However, the energy of this plane wave is $\mathcal{E}_\mu = -2t_A \cos\left(\frac{2\pi \mu F_{n-1}}{F_n}\right)$. It is straightforward to check that the $\mathcal{E}_\mu$ labelled by $\mu$ and the $E_m$ labelled by $m$ represent the same set of energies. They are simply ordered differently. The perpendicular space and real space wavenumbers can be related to each other (modulo $F_n$) by equating $E_m$ and $\mathcal{E}_\mu$
\begin{align}\label{eq:mcongruentmuApp}
    m \equiv \mu F_{n-1} \pmod{F_n}
\end{align}
Bearing in mind that we will shortly introduce a perturbation with an $F_n$-site supercell, we describe the band structure of $\hat{H}_0$ as consisting of $F_n$ bands in a Brillouin zone that spans the interval $k\in\left[-\frac{\pi}{F_n},\frac{\pi}{F_n}\right[$. For the unperturbed problem, all the bands touch each other, reflecting the fact that we have done nothing other than downfold the usual $\cos\left(\frac{2 \pi k}{F_n}\right)$ dispersion onto a smaller Brillouin zone. Introducing the perturbation $\hat{\mathcal{H}}_w$ splits the doubly degenerate states of $\hat{\mathcal{H}}_0$, and opens $F_n - 1$ gaps. The gap opening can be seen using first-order perturbation theory. The edges of gaps with an even (odd) number of states below them are at $k = 0\left(\frac{\pi}{F_n}\right)$. We will show the calculation for the even case in detail. The odd case is entirely analogous.

The rank 2 degenerate subspace labelled by $\mu$ has two states $\ket{\mu, \pm}$ with energy $-2t_A\cos\left(\frac{2\pi F_{n-1}}{F_n}\mu\right)$. The first order
corrections are given by the eigensystem of a $2\times 2$ matrix $\hat{V}$ whose entries are $V_{\alpha\beta} = \bra{\mu,\alpha}\hat{\mathcal{H}}_w\ket{\mu,\beta}$ with $\alpha,\beta = \pm$.
% \begin{align}
% V_{++} & = & \ \begin{pmatrix}
% 1 & e^{-2\pi i\frac{\mu}{F_{n}}} & \dotsc  & e^{-2\pi i\frac{( F_{n} -1) \mu}{F_{n}}}
% \end{pmatrix}
% % \begin{pmatrix}
% % 0&&-2w&&\\
% % &\searrow&&\searrow\\
% % &&&&\\
% % -2w&&&&\\
% % &\searrow&&&\\
% % &&&&
% % \end{pmatrix}
% \hat{\mathcal{H}}_w
% \begin{pmatrix}
% 1\\
% e^{2\pi i\frac{\mu}{F_{n}}}\\
% \vdots \\
% e^{2\pi i\frac{( F_{n} -1) \mu}{F_{n}}}
% \end{pmatrix}\nonumber \\
%  & = & \ \begin{pmatrix}
% 1 & e^{-2\pi i\frac{\mu}{F_{n}}} & \dotsc  & e^{-2\pi i\frac{( F_{n} -1) \mu}{F_{n}}}
% \end{pmatrix}\begin{pmatrix}
% -2w\ e^{2\pi i\frac{F_{n-1} \mu}{F_{n}}}\\
% \vdots \\
% -2w\ e^{2\pi i\frac{( F_{n} -1) \mu}{F_{n}}}\\
% 0\\
% \vdots \\
% 0\\
% -2w\ 1\\
% \vdots \\
% -2w\ e^{2\pi i\frac{( F_{n-2} -1) \mu}{F_{n}}}
% \end{pmatrix}\nonumber\\
%  & = & -2w\ F_{n-2}\left( e^{2\pi i\frac{F_{n-1} \mu}{F_{n}}} \ +\ e^{-2\pi i\frac{F_{n-1} \mu}{F_{n}}}\right)\nonumber \\
%  & = & -4w\ F_{n-2}\cos\left( 2\pi\frac{F_{n-1} }{F_{n}}\mu\right)
% \end{align}
% The other terms are similarly computed resulting in 
\begin{align}
    V_{\alpha\beta} = \frac{-4w}{F_{n}}\begin{pmatrix}
F_{n-2}\cos\left( 2\pi\frac{F_{n-1} \mu}{F_{n}}\right) & \frac{\sin\left( 2\pi\frac{\mu}{F_{n}} F_{n-2}\right)}{\sin\left( 2\pi\frac{\mu}{F_{n}}\right)}\\
\frac{\sin\left( 2\pi\frac{\mu}{F_{n}} F_{n-2}\right)}{\sin\left( 2\pi\frac{\mu}{F_{n}}\right)} & F_{n-2}\cos\left( 2\pi\frac{F_{n-1} \mu}{F_{n}}\right)
\end{pmatrix}
\end{align}
The eigenvalues of $\displaystyle V_{\alpha\beta}$ are $\displaystyle \epsilon ^{\pm } =\frac{-4w}{F_{n}}\left[ F_{n-2}\cos\left( 2\pi\frac{F_{n-1} \mu}{F_{n}}\right) \pm \frac{\sin\left( 2\pi\frac{\mu}{F_{n}} F_{n-2}\right)}{\sin\left( 2\pi\frac{\mu}{F_{n}}\right)}\right]$, and the corresponding eigenvectors are $\displaystyle \left(\frac{1}{\sqrt{2}} ,\pm \ \frac{1}{\sqrt{2}}\right) \ $. So, we have that the plane waves with the wavenumber $\frac{2\pi \mu}{F_{n}}$ split into the states $\ket{\mu,\pm}^*$ with the energies $\mathcal{E}^{\pm}_\mu$
\begin{align}
    \mathcal{E}_\mu^{\pm} =& -\left( 2t_{A} + 4w\frac{F_{n-2}}{F_{n}}\right) \cos\left(\frac{2\pi F_{n-1}}{F_{n}}\mu\right) \nonumber\\
    &\mp \frac{4w}{F_{n}} \frac{\sin\left( 2\pi \frac{F_{n-2}}{F_{n}}\mu\right)}{\sin\left( \frac{2\pi }{F_{n}}\mu\right)}\label{eq:pert_eps:S}\\
    \braket{j|\mu,+}^* =& \sqrt{\frac{2}{F_n}}\cos\left(\frac{2\pi \mu j}{F_n}\right),
    \braket{j|\mu,-}^* = \sqrt{\frac{2}{F_n}}\sin\left(\frac{2\pi \mu j}{F_n}\right) \label{eq:pert_vec:S}
\end{align} 
By combining the gap labelling theorem and \eqref{eq:mcongruentmuApp}, we can compute the perpendicular space wavenumber of the slightly perturbed plane waves around each gap. $E_m$ is monotonic when $m \in [0,\lfloor F_n/2\rfloor]$. Therefore, for gaps with an even number of states below them
\begin{align}\label{eq:mtoqeven}
    &2m \equiv q F_{n-1} \equiv 2\mu F_{n-1} \pmod{F_{n}}\nonumber \\
    \implies& \mu =\frac{c F_n + q}{2}
\end{align}
where $c$ is some integer. For gaps with an odd number of states below them, an analogous calculation at the edge of the Brillouin zone \footnote{Using the convention that the eigenstate at the edge of the Brillouin zone with label $\mu$ has the wavenumber $\frac{2\pi (\mu + 1/2)}{F_n}$} results in:
\begin{align}\label{eq:mtoqodd}
    &2m+1 \equiv q F_{n-1} \equiv (2\mu+1) F_{n-1} \pmod{F_{n}}\nonumber\\
    \implies& \mu =\frac{c F_n + q-1}{2}
\end{align}


\section{Robustness of the charge oscillations}
\label{sec:Rob_app}
As mentioned in the main text, the oscillations of the charge density in perpendicular space are robust against local perturbations of the hopping integrals. The robustness of a particular oscillation at a gap $|q|$ is further found to scale inversely with the gap size $\Delta_{|q|}$, i.e., oscillatory features are lost for lower disorder strength in smaller gaps. In Fig.~\ref{fig:disorder_35}, we illustrate this qualitatively by the charge oscillations in the gaps $|q|=3$ and $|q|=5$, where $\Delta_{|q|=5} < \Delta_{|q|=3}$. For the gap with label $|q| = 3$, we find that the oscillations are fully visible upon introducing disorder of strength $\delta t/t = 0.2$, whereas oscillatory features are lost in the case $\delta t/t = 0.5$. For the $|q|=5$ gap, a disorder strength of $\delta t/t = 0.2$ is sufficient to wash out the five-period structure visible in the clean case, hence being less resilient to noise due to its smaller gap size.

\begin{figure}
    \centering
    \includegraphics[width = \columnwidth]{disorder_q3_q5.pdf} 
    % \includegraphics[width = 0.26\textwidth]{q3TemperatureFourier.pdf}
%     \resizebox{0.3\textwidth}{!}{
% \begin{tikzpicture}
%     \input{Tiks_Experimental_Setup}
% \end{tikzpicture}}
    \caption{Perpendicular space charge density for the disordered Fibonacci approximant at gaps with labels $|q|=3,5$ and varying disorder strength. Disorder averages are taken over 2000 realizations, the light background in the plots indicating the statistical error to the mean.}
    \label{fig:disorder_35}
\end{figure}
